BackdoorBench: A Comprehensive Benchmark and Analysis of Backdoor Learning

As an emerging approach to explore the vulnerability of deep neural networks (DNNs), backdoor learning has attracted increasing interest in recent years, and many seminal backdoor attack and defense algorithms are being developed successively or concurrently, in the status of a rapid arms race. However, mainly due to the diverse settings, and the difficulties of implementation and reproducibility of existing works, there is a lack of a unified and standardized benchmark of backdoor learning, causing unfair comparisons or unreliable conclusions (e.g., misleading, biased or even false conclusions). Consequently, it is difficult to evaluate the current progress and design the future development roadmap of this literature. To alleviate this dilemma, we build a comprehensive benchmark of backdoor learning called BackdoorBench. Our benchmark makes three valuable contributions to the research community. 1) We provide an integrated implementation of state-of-the-art (SOTA) backdoor learning algorithms (currently including 20 attack and 32 defense algorithms), based on an extensible modular-based codebase. 2) We conduct comprehensive evaluations with 5 poisoning ratios, based on 4 models and 4 datasets, leading to 11,492 pairs of attack-against-defense evaluations in total. 3) Based on above evaluations, we present abundant analysis from 10 perspectives via 18 useful analysis tools, and provide several inspiring insights about backdoor learning. We hope that our efforts could build a solid foundation of backdoor learning to facilitate researchers to investigate existing algorithms, develop more innovative algorithms, and explore the intrinsic mechanism of backdoor learning. Finally, we have created a user-friendly website at http://backdoorbench.com, which collects all important information of BackdoorBench, including codebase, docs, leaderboard, and model Zoo.

==> sections/analysis/dataset.tex <==
\subsection{Analysis of Dataset}
\label{sec: analysis of dataset}



==> sections/analysis/forgetting.tex <==
\subsection{Analysis of Forgetting}
\label{sec: analysis of forgetting}


\begin{figure*}[htbp]
\centering
\subfigure[BadNets, PreAct-ResNet18]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/forgetting/cifar10_badnet_preactresnet18_forget.png}
\end{minipage}%
}%
\subfigure[BadNets, VGG19]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/forgetting/cifar10_badnet_vgg19_bn_forget.png}
\end{minipage}%
}%

\subfigure[Blended, PreAct-ResNet18]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/forgetting/cifar10_blended_preactresnet18_forget.png}
\end{minipage}
}%
\subfigure[Blended, VGG19]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/forgetting/cifar10_blended_vgg19_bn_forget.png}
\end{minipage}
}%

\subfigure[SIG, PreAct-ResNet18]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/forgetting/cifar10_sig_preactresnet18_forget.png}
\end{minipage}
}%
\subfigure[SIG, VGG19]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/forgetting/cifar10_sig_vgg19_bn_forget.png}
\end{minipage}
}%

\subfigure[SSBA, PreAct-ResNet18]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/forgetting/cifar10_ssba_preactresnet18_forget.png}
\end{minipage}
}%
\subfigure[SSBA, VGG19]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/forgetting/cifar10_ssba_vgg19_bn_forget.png}
\end{minipage}
}%

\subfigure[TrojanNN, PreAct-ResNet18]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/forgetting/cifar10_trojannn_preactresnet18_forget.png}
\end{minipage}
}%
\subfigure[TrojanNN, VGG19]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/forgetting/cifar10_trojannn_vgg19_bn_forget.png}
\end{minipage}
}%
\centering
\caption{Distributions of forgetting events of benign training samples and poisoned samples in CIFAR-10 with PreAct-Resnet18 and VGG19. The upper title of each subfigure denotes the poisoning ratio, clean accuracy and attack success rate.}
\label{fig: forgetting_cifar10}
\end{figure*}

% ============================================================

\begin{figure*}[htbp]
\centering
\subfigure[BadNets, PreAct-ResNet18]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/forgetting/cifar100_badnet_preactresnet18_forget.png}
\end{minipage}%
}%
\subfigure[BadNets, VGG19]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/forgetting/cifar100_badnet_vgg19_bn_forget.png}
\end{minipage}%
}%

\subfigure[Blended, PreAct-ResNet18]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/forgetting/cifar100_blended_preactresnet18_forget.png}
\end{minipage}
}%
\subfigure[Blended, VGG19]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/forgetting/cifar100_blended_vgg19_bn_forget.png}
\end{minipage}
}%

\subfigure[SIG, PreAct-ResNet18]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/forgetting/cifar10_sig_preactresnet18_forget.png}
\end{minipage}
}%
\subfigure[SIG, VGG19]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/forgetting/cifar10_sig_vgg19_bn_forget.png}
\end{minipage}
}%

\subfigure[SSBA, PreAct-ResNet18]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/forgetting/cifar100_ssba_preactresnet18_forget.png}
\end{minipage}
}%
\subfigure[SSBA, VGG19]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/forgetting/cifar100_ssba_vgg19_bn_forget.png}
\end{minipage}
}%

\subfigure[TrojanNN, PreAct-ResNet18]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/forgetting/cifar100_trojannn_preactresnet18_forget.png}
\end{minipage}
}%
\subfigure[TrojanNN, VGG19]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/forgetting/cifar100_trojannn_vgg19_bn_forget.png}
\end{minipage}
}%
\centering
\caption{Distributions of forgetting events of benign training samples and poisoned samples in CIFAR-100 with PreAct-Resnet18 and VGG19. The upper title of each subfigure denotes the poisoning ratio, clean accuracy and attack success rate.}
\label{fig: forgetting_cifar100}
\end{figure*}

From the analysis of fast backdoor learning in Section~\ref{sec: quick learning} above, we gain the impression that the backdoor model rapidly and consistently memorizes poisoned samples. To further understand the internal mechanisms of backdoor learning, we adopt the concept of \textit{forgetting event}~\cite{forgetting} to characterize the learning dynamics during the training process. Specifically, a forgetting event is recorded when a training sample correctly predicted in the current epoch is incorrectly predicted in the next epoch. In this section, we calculate the number of forgetting events for both benign and poisoned training samples under different settings. The results on CIFAR-10 and CIFAR-100 are shown in Figure~\ref{fig: forgetting_cifar10} and Figure~\ref{fig: forgetting_cifar100}, respectively. It can be observed that the number of forgetting events for benign training samples follows an exponential distribution under the most settings. For poisoned training samples, we find that for most attacks (Blended, SIG, SSBA, TrojanNN), the higher the ASR (Attack Success Rate), the higher the proportion of samples with low forgetting events. However, BadNets exhibit the opposite behavior. The above observations are compatible with our high-level observation that the backdoor attack with higher poisoning ratios could quickly learn the stable mapping from the poisoned samples to the target class. Moreover, the forgetting event provides a fine-grained tool to analyze the contribution of each individual training sample, which could facilitate the development of more advanced backdoor attack and defense methods. 


==> sections/analysis/individual_attack_method.tex <==
\paragraph{Analysis of sensitivity}
\label{sec: analysis of individual_attack_method}
In this section, we investigate the sensitivity of various attack and defense methods, taking into consideration different related hyper-parameters. Although a part of these hyper-parameters has been analysed, we analyse these parameters from a global perspective, such as the strength of the trigger, and the interaction of multiple parameters. 

\textbf{Analysis of each individual attack algorithm}
We experiment on the CIFAR-10 dataset with Preact-Resnet18 and adjust one or two critical hyper-parameters with different poisoning ratios. 
% However, as hyper-parameter changes do not affect their ASR under this poisoning ratio, we further analyze their attack effects at alternate poisoning ratios. 
The results are illustrated in Figure~\ref{fig:sensiticity_attack}.

The strength of the trigger has a strong impact on the ASR for each backdoor attack, including the patch size of BadNets~\cite{gu2019badnets}, the blending ratio of Blended~\cite{chen2017targeted} and so on. For BPP~\cite{wang2022bppattack}, we manipulate the number of bits in the squeezed color palette within the range of 3 to 7. A lower number of bits implies a greater change in the original image, leading to an elevated ASR. For LC~\cite{turner2019labelconsistent}, we adjust its reduced amplitude between 0.1 and 1, which controls the trigger visibility. When the reduced amplitude falls below 0.2, the ASR decreases significantly. These very strong triggers mean that more changes are made to the original drawing, which is easier for the model to learn, resulting in stronger generalization performance.

The interaction results of hyper-parameters are a little more complex. Although each parameter directly or indirectly affects the strength of the trigger, the strength of the influence of different triggers is different. For Input-Aware~\cite{nguyen2020input} and SIG~\cite{SIG}, the effect of hyper-parameter on ASR is more similar to that of an additive effect. In both cases, the ASR at one corner is higher and the ASR at the opposite corner is lower. For WaNet~\cite{nguyen2021wanet} and TrojanNN~\cite{liu2018trojaning}, there is a hyper-parameter that directly affects the ASR. Only when this hyper-parameter reaches a certain level, the ASR will be relatively high and another hyper-parameter may have an impact on the backdoor attack. The grid size of WaNet~\cite{nguyen2021wanet} and The number of trojaned neurons for TrojanNN~\cite{liu2018trojaning} contributes to the attack.

\textbf{Analysis of Each Individual Defense Method}


% The ASR for each method is assessed based on the CIFAR-10 dataset. For the majority of these attack methods, we maintain a poisoning ratio of 5\% and adjust one or two critical hyper-parameters. However, as hyper-parameter changes do not affect their ASR under this poisoning ratio, we further analyze their attack effects at alternate poisoning ratios. The results are illustrated in Figure~\ref{fig:sensiticity_attack}.
% In the case of BadNets~\cite{gu2019badnets}, we increase the patch size from 1 to 5 and observe an upward trend with the increase in patch size. 
% For Blended~\cite{chen2017targeted}, we escalate the blending ratio between 0.01 and 0.4, which reveals that a larger blending ratio corresponds to an increased ASR.
% For BPP~\cite{wang2022bppattack}, we manipulate the number of bits in the squeezed color palette within the range of 3 to 7. A lower number of bits implies a greater change in the original image, leading to an elevated ASR.
% For LC~\cite{turner2019labelconsistent}, we adjust its reduced amplitude between 0.1 and 1, which controls the trigger visibility. The attack remains effective at a poison ratio of 0.5\% when the reduced amplitude is above 0.2. However, when the reduced amplitude falls below 0.2, the ASR decreases significantly.
% For Input-Aware~\cite{nguyen2020input}, we vary its mask density within the range of 0.016-0.128 and the weighting parameter $\lambda_{div}$ between 0.25 to 4. The results show that these two hyper-parameters notably influence the effectiveness of the attack.
% For SIG~\cite{SIG}, we change the trigger’s frequency between 2 and 10 and strength $\Delta$ between 10 and 80. Larger frequency and strength $\Delta$ values imply a more potent attack and thus a higher ASR.
% For WaNet~\cite{nguyen2021wanet}, we investigate the effects of warping hyper-parameters: the strength s ranging from 2 to 10 and the grid size k ranging from 0.2 to 1. As s and k decrease, the poisoned image closely resembles the original one, and consequently, results in a lower ASR.
% For TrojanNN~\cite{liu2018trojaning}, we allow the trigger size to vary from 1 to 5 and the number of trojaned neurons from 1 to 5. An increase in the number of trojaned neurons contributes to a higher ASR, while the trigger size has a marginal impact on the attack's effectiveness.


\begin{figure*}[htbp]
\centering
\includegraphics[width=\textwidth]{figs/sensitivity/sensitivity_attack.png}
\caption{The effects of attack methods under different hyper-parameters on CIFAR-10 with PreAct-ResNet18. For attacks where two hyper-parameters are adjusted, each axis represents a distinct hyper-parameter and ASR is marked in each box, the color of the box represents the level of ASR.}
\label{fig:sensiticity_attack}
\end{figure*}


\comment{
badnet
patch size: 1, 2, 3, 4, 5

blended
train & test alpha 0.01 0.05 0.1 0.2 0.4

bpp 
squeeze num: 8, 16, 32, 64, 128

sig
delta 10, 20, 40, 60, 80
f 2, 4, 6, 8, 10

inputaware
lambda div 0.25, 0.5, 1, 2, 4
mask density 0.016, 0.032, 0.064, 0.096, 0.128

wanet
s  0.2, 0.4, 0.6, 0.8, 1
k  2, 4, 6, 8, 10

trojannn
num_neuron 1, 2, 3, 4, 5

lc
reduced_amplitude 0.2, 0.4, 0.6, 0.8, 1

LF and SSBA have no argument to be adjusted.
}

==> sections/analysis/individual_defense_method.tex <==
\subsection{Analysis of each individual defense algorithm}
\label{sec: analysis of individual_defense_method}

Some defense methods are sensitive to hyper-parameters and can achieve optimal results only under specific settings. In this section, we evaluate the performance of defense methods under different hyper-parameters on CIFAR-10, aiming to investigate their sensitivity. The poison ratio is set to 5\%. For each defense method, a pivotal hyper-parameter is chosen. The results are shown in Figure~\ref{fig: sensitivity_defense}.
For ABL~\cite{li2021anti} we choose the flooding value, setting it to values between 0.1 and 0.8, the results indicate that an appropriate flood ratio greatly impacts the defense effect.
ANP~\cite{wu2021adversarial} prunes neurons by a threshold, which we set within the range of 0.1 to 0.8. For most attacks, a larger threshold can significantly decrease the ASR, although a higher threshold might also lead to a decrease in clean accuracy.
For I-BAU~\cite{i-bau}, we adjust the number of rounds between 2 to 20. Within this range, I-BAU demonstrates relative stability. However, the defensive effectiveness can exhibit some variance for specific attacks, necessitating the selection of an appropriate hyper-parameter.
For NAD~\cite{nad-iclr-2020}, the distillation parameter $\beta$ is a key factor for NAD to successfully erase backdoor triggers. As $\beta$ increases, the ASR tends to decrease. However, when $\beta$ is excessively large, it may result in a decrease in the CA. Therefore, it is necessary to seek a balance.
For DBD~\cite{huang2022backdoor}, we choose the hyper-parameter $\epsilon$, which means the upper bound of the number of poisoned training samples. The results show that the selection of hyper-parameters also affects the defense effect.
For CLP~\cite{clp-2022}/EP/BNP~\cite{ep-bnp-2022}, we change the hyper-parameter u from 1 to 10, which controls the trade-off between ASR and CA. Results illustrate that it's crucial to appropriately select the value of u to realize the best performance of defense in these methods.
For FT, we change the ratio of clean data from 0.01 to 0.2. The results indicate that this modification can considerably influence the effectiveness of defense.

% 不用在这改了
% 我在别的地方重新写了，改图就好了


\begin{figure*}[htbp]
\centering
\subfigure[BadNets, PreAct-ResNet18, pratio=0.05]{
\begin{minipage}[t]{0.95\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/sensitivity/badnet_sensitivity.png}
\end{minipage}%
}%

\subfigure[Blended, PreAct-ResNet18, pratio=0.05]{
\begin{minipage}[t]{0.95\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/sensitivity/blended_sensitivity.png}
\end{minipage}%
}%


\centering
\caption{The effects of defense methods under different hyper-parameters on CIFAR-10 with PreAct-ResNet18.}
\label{fig: sensitivity_defense}
\end{figure*}



\comment{
clp
u 0-10

bnp
u 0-10

ep
u 0-10

anp 
threshold 0-0.9

abl  
flooding  0.1 0.2, 0.4, 0.6, 0.8 

i-bau
n_rounds 2, 4, 8, 16, 20

nad
beta3 50, 100, 500, 3000, 5000

dbd 
epsilon 0.1, 0.2, 0.4, 0.6, 0.8 

ft
ratio 0.01 0.05, 0.08, 0.1, 0.2

}

==> sections/analysis/quick_learning.tex <==
\subsection{Quick Learning}
\label{sec: quick learning}

The quick learning phenomenon of backdoor is the key problem to explore the learning ability of backdoor. \cite{abl} has used the fast learning phenomenon to distinguish clean and backdoor samples and mitigate the influence of backdoor. In the following, we provide a detailed analysis from the perspective of gradient. Specifically, for each epoch during the training process, we record the following information: 
      \begin{itemize}
        \item Losses of training samples, clean training samples, and poisoned training samples;
        \item Accuracy on training samples, clean training samples, and poisoned training samples;
        \item Gradient signal to noise ratios (GSNR) \cite{liu2020understanding} on training samples, clean train samples, and poisoned training samples averaged over model parameters;
        \item Norms of average gradient on total training samples, clean training samples, and poisoned training samples;
        \item Pairwise cosine similarities between average gradients on total training samples, clean training samples, and poisoned training samples.
    \end{itemize}
\begin{figure*}[htbp]
\centering
\subfigure[BadNets, PreAct-ResNet18 pratio=0.1]{
\begin{minipage}[t]{0.9\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/quick_learn/cifar10_preactresnet18_badnet_0_1_quick_learn.pdf}
\end{minipage}%
}%

\subfigure[BadNets, PreAct-ResNet18 pratio=0.01]{
\begin{minipage}[t]{0.9\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/quick_learn/cifar10_preactresnet18_badnet_0_01_quick_learn.pdf}
\end{minipage}%
}%

\subfigure[BadNets, PreAct-ResNet18 pratio=0.001]{
\begin{minipage}[t]{0.9\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/quick_learn/cifar10_preactresnet18_badnet_0_001_quick_learn.pdf}
\end{minipage}%
}%

\centering
\subfigure[Blended, PreAct-ResNet18 pratio=0.1]{
\begin{minipage}[t]{0.9\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/quick_learn/cifar10_preactresnet18_blended_0_1_quick_learn.pdf}
\end{minipage}%
}%

\subfigure[Blended, PreAct-ResNet18 pratio=0.01]{
\begin{minipage}[t]{0.9\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/quick_learn/cifar10_preactresnet18_blended_0_01_quick_learn.pdf}
\end{minipage}%
}%

\subfigure[Blended, PreAct-ResNet18 pratio=0.001]{
\begin{minipage}[t]{0.9\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/quick_learn/cifar10_preactresnet18_blended_0_001_quick_learn.pdf}
\end{minipage}%
}%

\subfigure[SIG, PreAct-ResNet18 pratio=0.01]{
\begin{minipage}[t]{0.9\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/quick_learn/cifar10_preactresnet18_sig_0_01_quick_learn.pdf}
\end{minipage}%
}%

\subfigure[SIG, PreAct-ResNet18 pratio=0.001]{
\begin{minipage}[t]{0.9\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/quick_learn/cifar10_preactresnet18_sig_0_001_quick_learn.pdf}
\end{minipage}%
}%

\centering
\subfigure[LF, PreAct-ResNet18 pratio=0.1]{
\begin{minipage}[t]{0.9\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/quick_learn/cifar10_preactresnet18_lf_0_1_quick_learn.pdf}
\end{minipage}%
}%

\subfigure[LF, PreAct-ResNet18 pratio=0.01]{
\begin{minipage}[t]{0.9\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/quick_learn/cifar10_preactresnet18_lf_0_01_quick_learn.pdf}
\end{minipage}%
}%

\subfigure[LF, PreAct-ResNet18 pratio=0.001]{
\begin{minipage}[t]{0.9\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/quick_learn/cifar10_preactresnet18_lf_0_001_quick_learn.pdf}
\end{minipage}%
}%

\centering
\subfigure[SSBA, PreAct-ResNet18 pratio=0.1]{
\begin{minipage}[t]{0.9\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/quick_learn/cifar10_preactresnet18_ssba_0_1_quick_learn.pdf}
\end{minipage}%
}%

\subfigure[SSBA, PreAct-ResNet18 pratio=0.01]{
\begin{minipage}[t]{0.9\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/quick_learn/cifar10_preactresnet18_ssba_0_01_quick_learn.pdf}
\end{minipage}%
}%

\subfigure[SSBA, PreAct-ResNet18 pratio=0.001]{
\begin{minipage}[t]{0.9\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/quick_learn/cifar10_preactresnet18_ssba_0_001_quick_learn.pdf}
\end{minipage}%
}%

\centering
\subfigure[Trojannn, PreAct-ResNet18 pratio=0.1]{
\begin{minipage}[t]{0.9\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/quick_learn/cifar10_preactresnet18_trojannn_0_1_quick_learn.pdf}
\end{minipage}%
}%

\subfigure[Trojannn, PreAct-ResNet18 pratio=0.01]{
\begin{minipage}[t]{0.9\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/quick_learn/cifar10_preactresnet18_trojannn_0_01_quick_learn.pdf}
\end{minipage}%
}%

\subfigure[Trojannn, PreAct-ResNet18 pratio=0.001]{
\begin{minipage}[t]{0.9\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/quick_learn/cifar10_preactresnet18_trojannn_0_001_quick_learn.pdf}
\end{minipage}%
}%

\centering
\caption{Accuracy, loss and gradient-related information of backdoor and clean samples during training under different attack and different poison ratios.}
\label{fig: quick_learn_sum}
\end{figure*}



In the figure, we show the relevant information of training samples in the training process under the conditions of \red{different attack} and \red{different poison ratio} using the PreAct-ResNet18 model under the CIFAR10 data set. From the figure, we can see that the poison sample gradient information of all backdoor attacks in the third column is much larger than that of the clean sample, and it is constantly decreasing. In the fourth column, the gradient information content (GSNR) of the backdoor sample is much higher than that of the clean sample, especially the lower the pratio, the higher the information density of the backdoor sample. We can assume that information from backdoor samples is more easily recognized than that from clean samples. At the same time, we can see from the figure that when the poison ratio is fixed, the fast learning phenomenon of the backdoor is continuously enhanced with the continuous increase of attack intensity. For example, when the blending degree increases from 0.1-0.2, we find that the train loss of backdoor sample decreases faster and faster. In summary, we believe that the fast learning of the backdoor is highly correlated with the proportion and intensity of poisoning.

% However, from the table of training loss and training accuracy, we can find that when the trigger of the attack is large and the poisoning rate is high, such as for blended, sig, trojann and other attacks, the loss of backdoor sample decreases faster than that of clean sample, and the backdoor sample is easier to be remembered. But in other cases, backdoor sample losses decline much more slowly than clean sample losses and cannot be better learned by the model.

\begin{figure*}[htbp]

\centering
\subfigure[Blended, PreAct-ResNet18 pratio=0.01, Blending ratio=0.1]{
\begin{minipage}[t]{0.9\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/quick_learn/cifar10_preactresnet18_blended_0_01_quick_learn_0_1.pdf}
\end{minipage}%
}%

\subfigure[Blended, PreAct-ResNet18 pratio=0.01, Blending ratio=0.15]{
\begin{minipage}[t]{0.9\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/quick_learn/cifar10_preactresnet18_blended_0_01_quick_learn_0_15.pdf}
\end{minipage}%
}%

\subfigure[Blended, PreAct-ResNet18 pratio=0.01, Blending ratio=0.2]{
\begin{minipage}[t]{0.9\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/quick_learn/cifar10_preactresnet18_blended_0_01_quick_learn_0_2.pdf}
\end{minipage}%
}%

\centering
\subfigure[SIG, PreAct-ResNet18 pratio=0.01, Delta=5]{
\begin{minipage}[t]{0.9\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/quick_learn/cifar10_preactresnet18_sig_0_01_quick_learn_5.pdf}
\end{minipage}%
}%

\subfigure[SIG, PreAct-ResNet18 pratio=0.01, Delta=20]{
\begin{minipage}[t]{0.9\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/quick_learn/cifar10_preactresnet18_sig_0_01_quick_learn_20.pdf}
\end{minipage}%
}%

\subfigure[SIG, PreAct-ResNet18 pratio=0.01, Delta=40]{
\begin{minipage}[t]{0.9\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/quick_learn/cifar10_preactresnet18_sig_0_01_quick_learn_40.pdf}
\end{minipage}%
}%

\centering
\subfigure[Trojannn, PreAct-ResNet18 pratio=0.01, Blending ratio=0.2]{
\begin{minipage}[t]{0.9\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/quick_learn/cifar10_preactresnet18_trojannn_0_01_quick_learn_0_2.pdf}
\end{minipage}%
}%

\subfigure[Trojannn, PreAct-ResNet18 pratio=0.01, Blending ratio=0.6]{
\begin{minipage}[t]{0.9\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/quick_learn/cifar10_preactresnet18_trojannn_0_01_quick_learn_0_6.pdf}
\end{minipage}%
}%

\subfigure[Trojannn, PreAct-ResNet18 pratio=0.01, Blending ratio=1.0]{
\begin{minipage}[t]{0.9\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/quick_learn/cifar10_preactresnet18_trojannn_0_01_quick_learn_1_0.pdf}
\end{minipage}%
}%

\centering
\caption{Accuracy, loss and gradient-related information of backdoor and clean samples during training under different attack and different intensity.}
\label{fig: quick_learn_sum}
\end{figure*}

% ============================================================



% \begin{itemize}
%         \item Losses of training samples, clean testing samples, and poisoned testing samples;
%         \item Accuracy on training samples, clean testing samples, and poisoned testing samples;
%         \item Gradient signal to noise ratios (GSNR) \cite{liu2020understanding} on training samples, clean train samples, and poisoned training samples averaged over model parameters;
%         \item Norms of average gradient on total training samples, clean training samples, and poisoned training samples;
%         \item Pairwise cosine similarities between average gradients on total training samples, clean training samples, and poisoned training samples.
%     \end{itemize}


